End-to-End User Behavior Retrieval in Click-Through RatePrediction Model

Click-Through Rate (CTR) prediction is one of the core tasks in recommender systems (RS). It predicts a personalized click probability for each user-item pair. Recently, researchers have found that the performance of CTR model can be improved greatly by taking user behavior sequence into consideration, especially long-term user behavior sequence. The report on an e-commerce website shows that 23\% of users have more than 1000 clicks during the past 5 months. Though there are numerous works focus on modeling sequential user behaviors, few works can handle long-term user behavior sequence due to the strict inference time constraint in real world system. Two-stage methods are proposed to push the limit for better performance. At the first stage, an auxiliary task is designed to retrieve the top-$k$ similar items from long-term user behavior sequence. At the second stage, the classical attention mechanism is conducted between the candidate item and $k$ items selected in the first stage. However, information gap happens between retrieval stage and the main CTR task. This goal divergence can greatly diminishing the performance gain of long-term user sequence. In this paper, inspired by Reformer, we propose a locality-sensitive hashing (LSH) method called ETA (End-to-end Target Attention) which can greatly reduce the training and inference cost and make the end-to-end training with long-term user behavior sequence possible. Both offline and online experiments confirm the effectiveness of our model. We deploy ETA into a large-scale real world E-commerce system and achieve extra 3.1\% improvements on GMV (Gross Merchandise Value) compared to a two-stage long user sequence CTR model.

==> source/fig1.tex <==
% transformer 局部放大？
\tikzset{
  ffn/.style = {draw, rectangle, fill=yellow3, minimum width=3em, minimum height=1.5em},
  item/.style = {draw, rectangle, fill=blue1, minimum width=3em, minimum height=1.5em},
  smallitem/.style = {draw, rectangle, fill=blue0, minimum width=2.8em, minimum height=1.8em},
  pvector/.style = {draw, rectangle, fill=blue2, minimum width=2.8em, minimum height=1.8em},
  transformer/.style = {draw, rectangle, fill=padua, minimum width=3em, minimum height=1.5em},
  norm/.style = {draw, rectangle, fill=blue1, minimum width=5.5em, minimum height=1.2em, inner sep=0, outer sep=0},
  dropout/.style = {draw, rectangle, fill=blue2, minimum width=4.5em, minimum height=1.2em, inner sep=0, outer sep=0},
  mh/.style = {draw, rectangle, fill=yellow2, minimum width=5.0em, minimum height=2.0em},
  ff/.style = {draw, rectangle, fill=blue3, minimum width=4.5em, minimum height=1.5em},
  softmax/.style = {circle, draw, line width=0.5pt, minimum size=1.5em, inner sep=0pt, align=center},
  relu/.style = {draw, rectangle, fill=yellow3, minimum width=3.5cm, minimum height=0.5cm},
  concat/.style = {draw, rectangle, fill=yellow3, minimum width=15.0em, minimum height=0.5cm},
  relu2/.style = {draw, rectangle, fill=yellow2, minimum width=2.5cm, minimum height=0.5cm},
  sigmoid/.style = {draw, rectangle, fill=yellow1, minimum width=1.5cm, minimum height=0.5cm},
  pretrain_item1/.style = {draw, rectangle, fill=yellow4, minimum width=1.5cm, minimum height=0.5cm},
  pretrain_item2/.style = {draw, rectangle, fill=yellow3, minimum width=1.5cm, minimum height=0.5cm},
  pretrain_item3/.style = {draw, rectangle, fill=yellow2, minimum width=1.5cm, minimum height=0.5cm},
  seq0/.style = {draw, rectangle, fill=yellow0, minimum width=0.5cm, minimum height=0.5cm},
  seq1/.style = {draw, rectangle, fill=yellow1, minimum width=0.5cm, minimum height=0.5cm},
  seq2/.style = {draw, rectangle, fill=yellow2, minimum width=0.5cm, minimum height=0.5cm},
  seq3/.style = {draw, rectangle, fill=yellow3, minimum width=0.5cm, minimum height=0.5cm},
  seq4/.style = {draw, rectangle, fill=yellow4, minimum width=0.5cm, minimum height=0.5cm},
  seq5/.style = {draw, rectangle, fill=yellow5, minimum width=0.5cm, minimum height=0.5cm},
  seq6/.style = {draw, rectangle, fill=yellow6, minimum width=0.5cm, minimum height=0.5cm},
  emb0/.style = {draw, rectangle, fill=blue0, minimum width=0.5cm, minimum height=0.5cm},
  emb1/.style = {draw, rectangle, fill=blue1, minimum width=0.5cm, minimum height=0.5cm},
  emb2/.style = {draw, rectangle, fill=blue2, minimum width=0.5cm, minimum height=0.5cm},
  emb3/.style = {draw, rectangle, fill=blue3, minimum width=0.5cm, minimum height=0.5cm},
  emb4/.style = {draw, rectangle, fill=blue4, minimum width=0.5cm, minimum height=0.5cm},
  emb5/.style = {draw, rectangle, fill=blue5, minimum width=0.5cm, minimum height=0.5cm},
  emb6/.style = {draw, rectangle, fill=blue6, minimum width=0.5cm, minimum height=0.5cm},
}



% 本论文使用配色
%\definecolor{blue0}{RGB}{240,249,232}
%\definecolor{blue1}{RGB}{204,235,197}
%\definecolor{blue2}{RGB}{168,221,181}
%\definecolor{blue3}{RGB}{123,204,196}
%\definecolor{blue4}{RGB}{78,179,211}
%\definecolor{blue5}{RGB}{43,140,190}
%\definecolor{blue6}{RGB}{8,88,158}
%
%
%\definecolor{yellow0}{RGB}{255,255,212}
%\definecolor{yellow1}{RGB}{254,227,145}
%\definecolor{yellow2}{RGB}{254,196,79}
%\definecolor{yellow3}{RGB}{254,153,41}
%\definecolor{yellow4}{RGB}{236,112,20}
%\definecolor{yellow5}{RGB}{204,76,2}
%\definecolor{yellow6}{RGB}{140,45,4}


%portafino

\begin{figure}[htb]
\centering
\resizebox{0.45\textwidth}{!}{
\begin{tikzpicture}[]

 
 \pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)
% 全局的距离
\def\vdistance{1.2cm}
% 全局的绝对位置起点（-5，-5）


%%%%%%%%%%%%% 第二部分 %%%%%%%%%%5

% \draw[thick,dotted]  ($(pretrain_e1.south west)+(-0.5, -1.2)$) rectangle ($(pv.north east)+(0.3, 1.3)$);

\node[inner sep=0pt] (inb) at(0.0,0.0)
    {\includegraphics[width=18px,height=18px]{fig/tshirt.png}};
\node[inner sep=0pt, right of=inb, node distance=\vdistance] (i3b) {\includegraphics[width=18px,height=18px]{fig/hat10.png}};

\node[inner sep=0pt, right of=i3b, node distance=\vdistance] (i2b) {\includegraphics[width=18px,height=18px]{fig/t02.png}};

\node[right of=i2b, node distance=0.8cm] (i0b) {$\dots$};

\node[inner sep=0pt, right of=i0b, node distance=0.8cm] (i1b) {\includegraphics[width=18px,height=18px]{fig/shoe05.png}};

\node[inner sep=0pt, right of=i1b, node distance=2cm] (t1b) {\includegraphics[width=18px,height=18px]{fig/bag.png}};


% shoe 上面的embedding
\node[seq0, above of=inb, node distance=1.6cm] (s00b) {};
%\node[seq1, above of=s00b, node distance=0.5cm] (s01b) {};
\node[seq2, above of=s00b, node distance=0.5cm] (s02b) {};
\node[seq3, above of=s02b, node distance=0.5cm] (s03b) {};

% dress 上面的embedding
\node[seq0, above of=i3b, node distance=1.6cm] (s10b) {};
%\node[seq2, above of=s10b, node distance=0.5cm] (s11b) {};
\node[seq1, above of=s10b, node distance=0.5cm] (s12b) {};
\node[seq3, above of=s12b, node distance=0.5cm] (s13b) {};

% baby 上面的embedding
\node[seq3, above of=i2b, node distance=1.6cm] (s20b) {};
%\node[seq1, above of=s20b, node distance=0.5cm] (s21b) {};
\node[seq2, above of=s20b, node distance=0.5cm] (s22b) {};
\node[seq0, above of=s22b, node distance=0.5cm] (s23b) {};

% man 上面的embedding
\node[seq1, above of=i1b, node distance=1.6cm] (s30b) {};
%\node[seq0, above of=s30b, node distance=0.5cm] (s31b) {};
\node[seq2, above of=s30b, node distance=0.5cm] (s32b) {};
\node[seq3, above of=s32b, node distance=0.5cm] (s33b) {};


% target item emb
\node[emb0, above of=t1b, node distance=1.6cm] (ti0b) {};
%\node[emb1, above of=ti0b, node distance=0.5cm] (ti1b) {};
\node[emb2, above of=ti0b, node distance=0.5cm] (ti2b) {};
\node[emb3, above of=ti2b, node distance=0.5cm] (ti3b) {};
 
% 方框
% \draw[thick,dotted]  ($(s03b.north)+(-0.5, 0.8)$) rectangle ($(s33b.north)+(0.5, 1.5)$) (dotted);
 
 \node[fit={($(s03b.north)+(-0.5, 0.8)$) ($(s33b.north)+(0.5, 1.5)$)}, inner sep=0pt, draw=blue, thick, dotted, rounded corners=4pt] (rect) {};

% qkv的箭头
 \draw[-{Latex[length=2mm, width=1.2mm]}] ($(ti3b.north)$) -- +(0.0,0.3) -- +(-5.8, 0.3) -- +(-5.8,0.8) ;
 
 \draw[-{Latex[length=2mm, width=1.2mm]}] ($(ti3b.north)+(-4.6,0.3)$) -- +(0.0,0.5) ;
 
  \draw[-{Latex[length=2mm, width=1.2mm]}] ($(ti3b.north)+(-3.3,0.3)$) -- +(0.0,0.5) ;
  
   \draw[-{Latex[length=2mm, width=1.2mm]}] ($(ti3b.north)+(-1.8,0.3)$) -- +(0.0,0.5) ;

 \draw[-{Latex[length=1mm, width=0.8mm]}] ($(s03b.north)$) -- +(0.0,0.8) ;
 \draw[-{Latex[length=1mm, width=0.8mm]}] ($(s03b.north)+(0.0,0.5)$) -- +(-0.2,0.0) -- +(-0.2,0.3) ;
 
  \draw[-{Latex[length=1mm, width=0.8mm]}] ($(s13b.north)$) -- +(0.0,0.8) ;
 \draw[-{Latex[length=1mm, width=0.8mm]}] ($(s13b.north)+(0.0,0.5)$) -- +(-0.2,0.0) -- +(-0.2,0.3) ;
 
 
  \draw[-{Latex[length=1mm, width=0.8mm]}] ($(s23b.north)$) -- +(0.0,0.8) ;
 \draw[-{Latex[length=1mm, width=0.8mm]}] ($(s23b.north)+(0.0,0.5)$) -- +(-0.2,0.0) -- +(-0.2,0.3) ;
 
 
  \draw[-{Latex[length=1mm, width=0.8mm]}] ($(s33b.north)$) -- +(0.0,0.8) ;
 \draw[-{Latex[length=1mm, width=0.8mm]}] ($(s33b.north)+(0.0,0.5)$) -- +(-0.2,0.0) -- +(-0.2,0.3) ;
 
% 文字qkv
\node[] at ($(s03b.north)+(-0.2,1.0)$) {K};
\node[] at ($(s03b.north)+(0.0,1.0)$) {V};
\node[] at ($(s03b.north)+(0.2,1.0)$) {Q};

\node[] at ($(s13b.north)+(-0.2,1.0)$) {K};
\node[] at ($(s13b.north)+(0.0,1.0)$) {V};
\node[] at ($(s13b.north)+(0.2,1.0)$) {Q};

\node[] at ($(s23b.north)+(-0.2,1.0)$) {K};
\node[] at ($(s23b.north)+(0.0,1.0)$) {V};
\node[] at ($(s23b.north)+(0.2,1.0)$) {Q};

\node[] at ($(s33b.north)+(-0.2,1.0)$) {K};
\node[] at ($(s33b.north)+(0.0,1.0)$) {V};
\node[] at ($(s33b.north)+(0.2,1.0)$) {Q};
    
% target attention之后的emb

% shoe 上面的embedding
\node[seq0, above of=s03b, node distance=2.4cm] (s00c) {};
%\node[seq1, above of=s00c, node distance=0.5cm] (s01c) {};
\node[seq2, above of=s00c, node distance=0.5cm] (s02c) {};
\node[seq3, above of=s02c, node distance=0.5cm] (s03c) {};

% dress 上面的embedding
\node[seq0, above of=s13b, node distance=2.4cm] (s10c) {};
%\node[seq2, above of=s10c, node distance=0.5cm] (s11c) {};
\node[seq1, above of=s10c, node distance=0.5cm] (s12c) {};
\node[seq3, above of=s12c, node distance=0.5cm] (s13c) {};

% baby 上面的embedding
\node[seq3, above of=s23b, node distance=2.4cm] (s20c) {};
%\node[seq1, above of=s20c, node distance=0.5cm] (s21c) {};
\node[seq2, above of=s20c, node distance=0.5cm] (s22c) {};
\node[seq0, above of=s22c, node distance=0.5cm] (s23c) {};

% man 上面的embedding
\node[seq1, above of=s33b, node distance=2.4cm] (s30c) {};
%\node[seq0, above of=s30c, node distance=0.5cm] (s31c) {};
\node[seq2, above of=s30c, node distance=0.5cm] (s32c) {};
\node[seq3, above of=s32c, node distance=0.5cm] (s33c) {};


% weighted sum
\node[softmax, yshift=1.0cm] at ($(s13c)!0.5!(s23c)$) (weightedsum) {\huge $+$};

% sum之后的向量
\node[seq2,above of=weightedsum, node distance=1.0cm] (s32d) {};

\node[seq1, left of=s32d, node distance=0.5cm] (s30d) {};
%\node[seq0, right of=s30d, node distance=0.5cm] (s31d) {};

\node[seq3, right of=s32d, node distance=0.5cm] (s33d) {};

% 各种连接线
\draw[-{Latex[length=1mm, width=0.8mm]}] ($(s30c.south)+(0.0,-0.3)$) -- (s30c.south) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] ($(s20c.south)+(0.0,-0.3)$) -- (s20c.south) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] ($(s10c.south)+(0.0,-0.3)$) -- (s10c.south) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] ($(s00c.south)+(0.0,-0.3)$) -- (s00c.south) ;

\draw[-{Latex[length=1mm, width=0.8mm]}] (s33c.north) -- (weightedsum.south) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] (s23c.north) -- (weightedsum.south) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] (s13c.north) -- (weightedsum.south) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] (s03c.north) -- (weightedsum.south) ;

\draw[-{Latex[length=1mm, width=0.8mm]}] (weightedsum.north) -- ($(weightedsum.north)+(0.0,0.5)$) ;


%%%%%%%%%%%%% 第三部分 %%%%%%%%%%5
\node[] at ($(ti3b)+(1.0, 1.0)$) (3q)  {Q};
\node[right of=3q, node distance=2.0cm] (3k)  {K};
\node[right of=3k, node distance=2.0cm] (3v)  {V};
\node[relu2, yshift=1.0cm] at ($(3q)!0.5!(3k)$) (mat1)  {MatMul};

\node[relu2, above of=mat1, node distance=1.0cm] (soft)  {SoftMax};

\node[relu2, yshift=3.0cm] at ($(3k)!0.5!(3v)$) (mat2)  {MatMul};

% 箭头
\draw[-{Latex[length=1mm, width=0.8mm]}] (3q.north) -- ($(3q.north)+(0.0,0.5)$) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] (3k.north) -- ($(3k.north)+(0.0,0.5)$) ;
\draw[-{Latex[length=1mm, width=0.8mm]}] (3v.north) -- ($(3v.north)+(0.0,2.5)$) ;

\draw[-{Latex[length=1mm, width=0.8mm]}] (mat1.north) -- (soft.south) ;

\draw[-{Latex[length=1mm, width=0.8mm]}] ($(3k.north)+(0.0,2.0)$) -- ($(3k.north)+(0.0,2.5)$) ;

\draw[-{Latex[length=1mm, width=0.8mm]}] ($(mat2.north)+(0.0,0.0)$) -- ($(mat2.north)+(0.0,0.5)$) ;


% 图b的虚框
 \node[fit={($(3q.north west)+(-0.5, 4.0)$) ($(3v.south east)+(0.5, 0.0)$)}, inner sep=0pt, draw=blue, thick, dotted, rounded corners=4pt] (dottedrect) {};
 
\node[] at ($(3q.north west)+(2.2, 3.7)$) (text) {\LARGE Scaled Dot-Product Attention};

\draw[-{Latex[length=2mm, width=2.8mm]}, dotted,blue,line width=1mm] ($(rect.north east)+(0.0,0.0)$) -- ($(dottedrect.west)+(0.0,0.0)$) ;


\end{tikzpicture}
}
    \caption{Multi-head target attention. }
    \label{fig:model2}
\end{figure}
